Basis Manifold

In this paper we study a symmetry group of vector space. Basis manifold is a homogeneous space of a symmetry group. This concept leads us to the definition of active and passive transformations on basis manifold. Active transformation can be expressed as a transformation of vector space. Passive transformation gives ability to define concepts of invariance and of geometrical object.

==> Basis.Russian.tex <==
%auto-ignore
\def\texBasis{}
\ifx\PrintBook\undefined
\else
				\chapter{Многообразие базисов}
\fi

			\section{Базис в векторном пространстве}
			\label{section: Basis in Vector Space}

Пусть мы имеем векторное пространство \symb{\mathcal{V}}1{V}
и контравариантное правостороннее эффективное линейное
представление группы
\symb{G(\mathcal{V})}0{GV}
$G=\ShowSymbol{GV}$.
Мы обычно будем называть группу $G(\mathcal{V})$
\AddIndex{группой симметрии}{symmetry group}.
Не нарушая общности, мы будем отождествлять элемент $g$ группы $G$
с соответствующим преобразованием представления
и записывать его действие на вектор $v\in\mathcal{V}$
в виде $vg$.

Эта точка зрения позволяет определить два типа координат
для элемента $g$ группы $G$. Мы можем либо пользоваться координатами,
определёнными на группе, либо определить координаты как
элементы матрицы соответствующего преобразования.
Первая форма координат более эффективна, когда мы изучаем
свойства группы $G$. Вторая форма координат
содержит избыточную информацию, но бывает более удобна,
когда мы изучаем представление группы $G$.
Мы будем называть вторую форму координат
\AddIndex{координатами представления}{coordinates of representation}.

Мы будем называть максимальное множество
линейно независимых векторов
\symb{\Basis{e}}0{Basis e}
$\ShowSymbol{Basis e}=<e_{(i)}>$
\AddIndex{базисом}{Basis}.
В том случае, когда мы хотим явно указать, что это базис
пространства $\mathcal{V}$, мы будем пользоваться обозначением
\symb{\Basis{e}_\mathcal{V}}1{basis in V}.

Любой гомоморфизм векторного пространства отображает один базис в другой. 
Таким образом, мы можем распространить ковариантное представление группы симметрии
на множество базисов.
Мы будем
записывать действие элемента $g$ группы $G$ на базис $\Basis{e}$
в виде \symb{R(g)\Basis{e}}1{active transformation}.
Тем не менее, не всякие два базиса могут быть связаны
преобразованием группы симметрии
потому, что не всякое невырожденное линейное преобразование принадлежит
представлению группы $G$. Таким образом, множество базисов
можно представить как объединение орбит группы $G$.

Свойства базиса зависят от группы симметрии.
Мы можем выбрать базисы $\Basis{e}$, векторы которых находятся
в отношении, которое инвариантно относительно группы симметрии.
В этом случае все базисы из орбиты
$\mathcal{O}(\Basis{e},g\in G,R(g)\Basis{e})$
имеют векторы, которые удовлетворяют одному и тому же отношению.
Такой базис мы будем называть
\AddIndex{\Gbasis ом}{G-basis}.
В каждом конкретном случае мы должны доказать существование
базиса с искомыми свойствами. Если подобного типа базиса
не существует, мы можем выбрать произвольный базис.

	 \begin{definition}
	 \label{definition: basis manifold of vector space}
Мы будем называть орбиту $\mathcal{O}(\Basis{e},g\in G,R(g)\Basis{e})$
выбранного базиса $\Basis{e}$
\AddIndex{многообразием базисов
\symb{\mathcal{B}(\mathcal{V})}1{basis manifold of vector space}
векторного пространства}{basis manifold of vector space}
$\mathcal{V}$.
	 \qed
	 \end{definition}

		\begin{theorem}
		\label{theorem: basis manifold of vector space}
Представление группы $G$ на многообразии базисов
однотранзитивно.
		\end{theorem}
		\begin{proof}
Согласно определению \ref{definition: basis manifold of vector space}
любые два базиса связаны по крайней мере одним преобразованием
представления. Для доказательства теоремы достаточно показать,
что это преобразование определено однозначно.

Допустим элементы $g_1$, $g_2$ группы $G$ и базис $\Basis{e}$ таковы, что
	\begin{equation}
R_{g_1}\Basis{e}=R_{g_2}\Basis{e}
	\label{eq: two transformations on basis manifold, 1}
	\end{equation}
Из \eqref{eq: two transformations on basis manifold, 1} следует
	\begin{equation}
R_{g_2^{-1}}R_{g_1}\Basis{e}=R_{g_1g_2^{-1}}\Basis{e}=\Basis{e}
	\label{eq: two transformations on basis manifold, 2}
	\end{equation}
Так как любой вектор имеет единственное разложение
относительно базиса $\Basis{e}$, то из
\eqref{eq: two transformations on basis manifold, 2} следует,
что $R_{g_1g_2^{-1}}$ тождественное преобразование
векторного пространства $\mathcal{V}$. Так как представление
группы $G$ эффективно на векторном пространстве $\mathcal{V}$,
то $g_1=g_2$.
Отсюда следует утверждение теоремы.
		\end{proof}

Из теоремы \ref{theorem: basis manifold of vector space} следует,
что многообразие базисов $\mathcal{B}(\mathcal{V})$ является однородным пространством группы $G$.
Мы построили контравариантное правостороннее однотранзитивное линейное
представление группы $G$ на многообразии базисов.
Мы будем называть это представление
\AddIndex{активным представлением}{active representation},
а соответствующее преобразование на многообразие базисов
\AddIndex{активным преобразованием}{active transformation}
(\citeBib{Korn})
потому, что гомоморфизм векторного пространства породил это преобразование.

Согласно теореме \ref{theorem: single transitive representation of group},
так как многообразие базисов $\mathcal{B}(\mathcal{V})$ -
однородное пространство группы $G$,
мы можем определить на $\mathcal{B}(\mathcal{V})$
две формы координат, определённые на группе $G$.
В обоих случаях координаты базиса $\Basis{e}$ - это
координаты гомоморфизма, отображающего заданный базис $\Basis{e}_0$ в
базис $\Basis{e}$.
Координаты представления называются
\AddIndex{стандартными координатами базиса}
{standard coordinates of basis}.
Нетрудно показать, что стандартные координаты
\symb{e^i_k}1{standard coordinates of basis}
базиса $\Basis{e}$ при заданном значении $k$ являются
координатами вектора
\symb{\Vector e_k}0{vector of basis}
$\ShowSymbol{vector of basis}\in\Basis{e}$
относительно заданного базиса $\Basis{e}_0$.

Базис $\Basis{e}$ порождает координаты на $\mathcal{V}$.
В различных типах пространства это может быть сделано различным образом.
В аффинном пространстве, если вершина базиса является точкой $A$, то
точка $B$ имеет те же координаты, что и вектор $\overset{\longrightarrow}{AB}$
относительно базиса $\Basis{e}$.
В общем случае мы вводим координаты вектора как координаты
относительно выбранного базиса.
Использование только \Gspaceа означает использование специальных координаты на $\mathcal{A}_n$.
Для того, чтобы отличать их, мы будем называть их
\AddIndex{\Gcoords ами}{G-coordinates}.
Мы также будем называть пространство $\mathcal{V}$ с такими координатами
\AddIndex{\Gspace ом}{GSpace}.

Согласно теореме \ref{theorem: two representations of group}, на многообразии базисов существует другое
представление, перестановочное с пассивным.
Как мы видим из замечания \ref{remark: one representation of group}
преобразование этого
представления отличается от пассивного преобразования и не может быть сведено к
преобразованию пространства $\mathcal{V}$.
Чтобы подчеркнуть различие, это преобразование называется
\AddIndex{пассивным преобразованием}{passive transformation}
векторного пространства $\mathcal{V}$,
а представление называется
\AddIndex{пассивным представлением}{passive representation}.
Мы будем записывать пассивное преобразование базиса $\Basis{e}$,
порождённое элементом $g\in G$,
в виде \symb{L(g)\Basis{e}}1{passive transformation}.

			\subsection{Базис в аффинном пространстве}
			\label{sec:AffineSpace}

Мы отождествляем векторы аффинного пространства
\symb{\mathcal{A}_n}1{An}
с парой точек $\overset{\longrightarrow}{AB}$.
Все векторы, которые имеют общее начало $A$ порождают векторное пространство,
которое мы будем называть касательным векторным пространством $T_A\mathcal{A}_n$.

Топология, которую $\mathcal{A}_n$ наследует из отображения $\mathcal{A}_n\rightarrow R^n$,
позволяет нам изучать непрерывные преобразования пространства $\mathcal{A}_n$
и их производные. Более точно, производная
преобразования $f$ отображает векторное пространство $T_A\mathcal{A}_n$ в $T_{f(A)}\mathcal{A}_n$.
Если $f$ линейно, то его производная одна и та же в каждой точке.
Вводя координаты $A^1,...,A^n$ точки $A\in\mathcal{A}_n$, мы можем записать
линейное преобразование как
	\begin{align}
A'^i&=P^i_j A^j + R^i &\det P\ne 0
	\label{eq: AffineTransformation}
	\end{align}
Производная этого преобразования определена матрицей $\|P^i_j\|$
и не зависит от точки $A$. Вектор
$(R^1,...,R^n)$ выражает смещение в аффинном пространстве.
Множество преобразований \eqref{eq: AffineTransformation} - это группа Ли,
которую мы обозначим \symb{GL(\mathcal{A}_n)}1{GLAn}
и будем называть
\AddIndex{группой аффинных преобразований}{AffineTransformationGroup}.

		\begin{definition}
\AddIndex{Аффинный базис}{Affine Basis}
\symb{\Basis{e}=<O,\Vector e_i>}1{Affine Basis} - это множество
линейно независимых векторов $\Vector e_i=\overset{\longrightarrow}{OA_i}=(e^1_i,...,e^n_i)$
с общей начальной точкой $O=(O^1,...,O^n)$. \qed
		\end{definition}

		\begin{definition}
\AddIndex{Многообразие базисов \symb{\mathcal{B}(\mathcal{A}_n)}1{BAn}
аффинного пространства}{Basis Manifold, Affine Space} %\index{manifold of}
- это множество базисов этого пространства.
		\qed
		\end{definition}

Мы будем называть активное преобразование
\AddIndex{аффинным преобразованием}{affine transformation}.
Мы будем называть пассивное преобразование
\AddIndex{квазиаффинным преобразованием}{quasi affine transformation}.

Если мы не заботимся о начальной точке вектора, мы получим несколько отличный
тип пространства, которое мы будем называть центро-аффинным пространством
\symb{\mathcal{CA}_n}1{CAn}.
В центро-аффинном пространстве мы можем идентифицировать все
касательные пространства и обозначить их $T\mathcal{CA}_n$.
Если мы предположим, что начальная точка
вектора - это начало $O$ координатной системы в пространстве,
то мы можем отождествить любую
точку $A\in\mathcal{CA}_n$ с вектором $a=\overset{\longrightarrow}{OA}$. Это ведёт
к идентификации $\mathcal{CA}_n$ и $T\mathcal{CA}_n$.
Теперь преобразование - это просто отображение
	\begin{align*}
a'^i&=P^i_j a^j & \det P\ne 0
	\end{align*}
и такие преобразования порождают группу Ли $GL_n$.

		\begin{definition}
\AddIndex{Центро-аффинный базис}{Central Affine Basis}
\symb{\Basis{e}=<\Vector e_i>}1{Central Affine Basis} - это множество
линейно независимых векторов $\Vector e_i=(e^1_i,...,e^n_i)$. \qed
		\end{definition}

		\begin{definition}
\AddIndex{Многообразие базисов \symb{\mathcal{B}(\mathcal{CA}_n)}1{BCAn}
центро-аффинного пространства}{Basis Manifold, Central Affine Space}
- это множество базисов этого пространства. \qed
		\end{definition}

			\subsection{Базис в евклидовом пространстве}
			\label{subsection: EuclideSpace}

Когда мы определяем метрику в центро-аффинном пространстве, мы
получаем новую геометрию потому, что
мы можем измерять расстояние и длину вектора. Если метрика
положительно определена, мы будем называть пространство евклидовым
\symb{\mathcal{E}_n}1{En},
в противном случае мы будем называть пространство псевдоевклидовым
\symb{\mathcal{E}_{nm}}1{Enm}.

Преобразования, которые сохраняют длину,
образуют группу Ли $SO(n)$ для евклидова пространства и группу Ли $SO(n,m)$ для
псевдоэвклидова пространства, где $n$ и $m$ числа положительных
и отрицательных слагаемых в метрике.

		\begin{definition}
\AddIndex{Ортонормальный базис}{Orthonornal Basis}
\symb{\Basis{e}=<\Vector e_i>}1{Orthonornal Basis} - это множество
линейно независимых векторов $\Vector e_i=(e^1_i,...,e^n_i)$ таких, что длина
каждого вектора равна $1$ и различные векторы ортогональны.
		\qed
		\end{definition}

Существование ортогонального базиса доказывается с помощью
процесса ортогонализации Грама--Шмидта.

		\begin{definition}
\AddIndex{Многообразие базисов \symb{\mathcal{B}(\mathcal{E}_n)}1{BEn}
евклидова пространства}{Basis Manifold, Euclid Space}
- это множество ортонормальных базисов этого пространства.
		\qed
		\end{definition}

Мы будем называть активное преобразование
\AddIndex{движением}{movement transformation}.
Мы будем называть пассивное преобразование
\AddIndex{квазидвижением}{quasi movement}.

			\section{Геометрический объект}
			\label{section: Geometrical Object of vector space}

Активное преобразование изменяет базисы и векторы согласовано
и координаты вектора относительно базиса не меняются.
Пассивное преобразование меняет только базис, и это ведёт к изменению
координат вектора относительно базиса.

Допустим пассивное преобразование $L(a)\in G$, заданное матрицей
$(a^i_j)$, отображает
базис $\Basis{e}=<e_i>\in\mathcal{B}(\mathcal{V})$
в базис $\Basis{e}'=<e'_i>\in\mathcal{B}(\mathcal{V})$
	\begin{equation}
	\label{eq: active transformation of vector space}
e'_j=a^i_je_i
	\end{equation}
Допустим вектор $v\in\mathcal{V}$ имеет разложение
	\begin{equation}
	\label{eq: vector expansion in vector space, basis f}
v=v^ie_i
	\end{equation}
относительно базиса $\Basis{e}$ и имеет разложение
	\begin{equation}
	\label{eq: vector expansion in vector space, basis fprim}
v=v'^ie'_i
	\end{equation}
относительно базиса $\Basis{e}'$.
Из \eqref{eq: active transformation of vector space}
и \eqref{eq: vector expansion in vector space, basis fprim} следует, что
	\begin{equation}
	\label{eq: vector expansion in vector space, basis f, 1}
v=v'^ja^i_je_i
	\end{equation}
Сравнивая \eqref{eq: vector expansion in vector space, basis f}
и \eqref{eq: vector expansion in vector space, basis f, 1} получаем, что
	\begin{equation}
	\label{eq: coordinate transformation, 1}
v^i=v'^ja^i_j
	\end{equation}
Так как $a^i_j$ - невырожденная матрица, то
из \eqref{eq: coordinate transformation, 1} следует
	\begin{equation}
	\label{eq: coordinate transformation}
v'^i=v^ja^{-1}{}^i_j
	\end{equation}
Преобразование координат \eqref{eq: coordinate transformation}
не зависит от вектора $v$ или базиса $\Basis{e}$, а
определенно исключительно координатами вектора $v$
относительно базиса $\Basis{e}$.

Если мы фиксируем базис $\Basis{e}$, то множество координат
\symb{(v^i)}1{coordinates in vector space}
относительно этого базиса порождает векторное пространство
\symb{\tilde{\mathcal{V}}}1{coordinate vector space},
изоморфное векторному пространству $\mathcal{V}$.
Это векторное пространство называется
\AddIndex{координатным векторным пространством}{coordinate vector space},
а изоморфизм
\AddIndex{координатным изоморфизмом}{coordinate isomorphism}.
Мы будем обозначать
\symb{\Vector\delta_k=(\delta^i_k)}1
{image of vector e_k, coordinate vector space}
образ вектора $e_k\in\Basis{e}$ при этом изоморфизме.
		\begin{theorem}
		\label{theorem: coordinate transformations form representation, vector space}
Преобразования координат \eqref{eq: coordinate transformation}
порождают контравариантное правостороннее эффективное линейное
представление группы $G$, называемое
\AddIndex{координатным представлением}
{coordinate representation, vector space}.
		\end{theorem}
		\begin{proof}
Допустим мы имеем два последовательных пассивных преобразования
$L(a)$ и $L(b)$. Преобразование координат \eqref{eq: coordinate transformation}
соответствует пассивному преобразованию $L(a)$.
Преобразование координат
	\begin{equation}
	\label{eq: coordinate transformation, b}
v''^k=v'^ib^{-1}{}^k_i
	\end{equation}
соответствует пассивному преобразованию $L(b)$. Произведение
преобразований координат \eqref{eq: coordinate transformation}
и \eqref{eq: coordinate transformation, b} имеет вид
	\begin{equation}
	\label{eq: coordinate transformation, ba}
v''^k=v^ja^{-1}{}^i_jb^{-1}{}^k_i=v^j(ba)^{-1}{}^k_j
	\end{equation}
и является координатным преобразованием,
соответствующим пассивному преобразованию $L_{ba}$.
Это доказывает, что преобразования координат
порождают контравариантное правостороннее линейное
представление группы $G$.

Если координатное преобразование не изменяет векторы $\delta_k$,
то ему соответствует единица группы $G$, так как пассивное представление
однотранзитивно. Следовательно,
координатное представление эффективно.
		\end{proof}

Предположим,
что гомоморфизм группы $G$ в
группу пассивных преобразований
векторного пространства $\mathcal{W}$ согласован с группой симметрий
векторного пространства $\mathcal{V}$.
Это означает, что пассивному преобразованию $L(a)$ векторного пространства $\mathcal{V}$
соответствует пассивное преобразование $L(a)$ векторного пространства $\mathcal{W}$.
	\begin{equation}
	\label{eq: passive transformation of vector space W}
E'_\alpha=A^\beta_\alpha(a)E_\beta
	\end{equation}
Тогда координатное преобразование в $\mathcal{W}$ принимает вид
	\begin{equation}
	\label{eq: coordinate transformation, W}
w'^\alpha=w^\beta A(a^{-1})^\alpha_\beta=w^\beta A(a)^{-1}{}^\alpha_\beta
	\end{equation}

		\begin{definition}
		\label{definition: geometrical object, coordinate representation}
Мы будем называть орбиту
\symb{\mathcal{O}((w,\Basis{e}_\mathcal{V}),
a\in G,(wA(a)^{-1},L(a)\Basis{e}_\mathcal{V}))}2
{geometrical object, coordinate vector space}%
\AddIndex{геометрическим объектом в координатном представлении}
{geometrical object, coordinate vector space},
определённым в векторном пространстве $\mathcal{V}$.
Для любого базиса
$\Basis{e}'_\mathcal{V}=L(a)\Basis{e}_\mathcal{V}$
соответствующая точка \eqref{eq: coordinate transformation, W} орбиты  определяет
\AddIndex{координаты геометрического объекта}
{coordinates of geometrical object, coordinate vector space}
относительно базиса $\Basis{e}'_\mathcal{V}$.
		\qed
		\end{definition}

		\begin{definition}
		\label{definition: geometrical object}
Мы будем называть орбиту
\symb{\mathcal{O}((w,\Basis{e}_\mathcal{W},\Basis{e}_\mathcal{V}),
a\in G,(wA(a)^{-1},L(a)\Basis{e}_\mathcal{W},
L(a)\Basis{e}_\mathcal{V}))}2
{geometrical object, vector space}%
\AddIndex{геометрическим объектом}{geometrical object, vector space},
определённым в векторном пространстве $\mathcal{V}$.
Для любого базиса
$\Basis{e}'_\mathcal{V}=L(a)\Basis{e}_\mathcal{V}$
соответствующая точка \eqref{eq: coordinate transformation, W} орбиты  определяет
\AddIndex{координаты геометрического объекта}{coordinates of geometrical object, vector space}
относительно базиса $\Basis{e}'_\mathcal{V}$
и соответствующий вектор
\[
w=w'^\alpha E'_\alpha
\]
называется
\AddIndex{представителем геометрического объекта}
{representative of geometrical object, vector space}
в базисе $\Basis{e}'_\mathcal{V}$.
		\qed
		\end{definition}

Мы будем также говорить, что $w$ - это
\AddIndex{геометрический объект типа $A$}
{geometrical object of type A, vector space}

Так как геометрический объект - это орбита представления,
то согласно теореме \ref{theorem: proper definition of orbit}
определение геометрического объекта корректно.

Определение \ref{definition: geometrical object, coordinate representation}
строит геометрический объект в координатном пространстве.
Определение \ref{definition: geometrical object} предполагает,
что мы выбрали базис в векторном пространстве $\mathcal{W}$.
Это позволяет использовать 
вместо его координат.

		\begin{theorem}[\AddIndex{принцип инвариантности}
		{invariance principle, vector space}]
		\label{theorem: invariance principle}
Представитель геометрического объекта не зависит от выбора
базиса $\Basis{e}'_\mathcal{V}$.
		\end{theorem}
		\begin{proof}
Чтобы определить представителя геометрического объекта,
мы должны выбрать базис $\Basis{e}_\mathcal{V}$,
базис
$\Basis{e}_\mathcal{W}=(E_\alpha)$
и координаты геометрического объекта
$w^\alpha$. Соответствующий представитель геометрического
объекта имеет вид
\[
w=w^\alpha E_\alpha
\]
Базис $\Basis{e}'_\mathcal{V}$ связан с базисом
$\Basis{e}_\mathcal{V}$ пассивным преобразованием $L(a)$.
Согласно построению это порождает пассивное преобразование
\eqref{eq: passive transformation of vector space W}
и координатное преобразование
\eqref{eq: coordinate transformation, W}. Соответствующий
представитель геометрического объекта имеет вид
\[
w'=w'^\alpha E'_\alpha
=w^\beta A(a)^{-1}{}^\alpha_\beta A^\gamma_\alpha(a)E_\gamma
=w'^\beta E'_\beta=w
\]
Следовательно, представитель геометрического
объекта инвариантен относительно выбора базиса.
		\end{proof}

		\begin{definition}
		\label{definition: sum of geometrical objects}
Пусть
\[w_1=w_1^\alpha E_\alpha\]
\[w_2=w_2^\alpha E_\alpha\]
геометрические объекты одного и того же типа,
определённым в векторном пространстве $\mathcal{V}$.
Геометрический объект
\[w=(w_1^\alpha+w_2^\alpha)E_\alpha\]
называется \AddIndex{суммой
\[w=w_1+w_2\]
геометрических объектов}{sum of geometrical objects, vector space}
$w_1$ и $w_2$.
		\qed
		\end{definition}

		\begin{definition}
		\label{definition: product of geometrical object and constant}
Пусть
\[w_2=w_2^\alpha E_\alpha\]
геометрический объект,
определённый в векторном пространстве $\mathcal{V}$ над полем $F$.
Геометрический объект
\[w_2=(kw_1^\alpha) E_\alpha\]
называется \AddIndex{произведением
\[w_2=kw_1\]
геометрического объекта $w_1$ и константы $k\in F$}
{product of geometrical object and constant, vector space}.
		\qed
		\end{definition}

		\begin{theorem}
Геометрические объекты типа $A$,
определённые в векторном пространстве $\mathcal{V}$ над полем $F$,
образуют векторное пространство над полем $F$.
		\end{theorem}
		\begin{proof}
Утверждение теоремы следует из непосредственной проверки
свойств векторного пространства.
		\end{proof}


==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{texIntro}{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84 (1966)
}%

\BiblioItem{texGenRelativity}{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{texGenRelativity}{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{texAffine}{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{texAffine}{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric-affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{texAffine}{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{texAffine}{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\BiblioItem{texAffine}{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%

\BiblioItem{texAffine}{0405.027}
{
Aleks Kleyn,
Reference Frame in General Relativity,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2004)
}%

\BiblioItem{texTidal,texAffine}{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{texTidal,texNewton}{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{texNewton}{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{texNewton}{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric-affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{texLagrange}{Weinberg}
{
Steven Weinberg. The Quantum Theory of Fields. Cambridge university press.
}%

\BiblioItem{texLagrange}{Reinhardt}
{
Greiner Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{texLagrange}{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{texTidal}{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{texTidal}{0405.028}
{
Aleks Kleyn, Metric-Affine Manifold,
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2004)
}%

\BiblioItem{texTidal}{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

\BiblioItem{texTidal}{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{texReferenceFrame,texAlgebraBundle}{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{texAlgebraBundle,texDrcRepresentation}{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

%\BiblioItem{texBasis}{Shilov}
%{
%Г. Е. Шилов, Математический анализ,
%Функции нескольких вещественных переменных, части 1 - 2,
%М., Наука, 1972
%}%

\BiblioItem{texAffine,texRepresentation,texBasis,texDrcBasis,texVectorSpace,texLinearMap}
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem{texDrcBasis,texBasis}{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

%\BiblioItem{Kleyn} http://www.geocities.com/aleks\_kleyn/Derivative/Derivative.htm

\BiblioItem{texGenRelativity}{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{texGenRelativity}{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{texGenRelativity}{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{texGenRelativity}{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{texGenRelativity}{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{texGenRelativity}{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{texGenRelativity}{Muller}
{
Holger Muller et al.,
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators,
\href{http://prola.aps.org/searchabstract/PRL/v91/i2/e020401}{Phys. Rev. Lett. 91, 020401} (2003),
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2000)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{texGenRelativity,texTidal}{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{texBiring,texVectorSpace}{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{texBiring,texVectorSpace}
{q-alg-9705026}
{
I.Gelfand, V.Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{texVectorSpace}{Gelfand Retakh 1991}
{
I. Gelfand and V. Retakh, Determinants of Matrices over Noncommutative Rings, Funct.
Anal. Appl. 25 (1991), no. 2, 91-102
}%

\BiblioItem{texVectorSpace}{Gelfand Retakh 1992}
{
I. Gelfand and V. Retakh, A Theory of Noncommutative Determinants and Characteristic
Functions of Graphs, Funct. Anal. Appl. 26 (1992), no. 4, 1-20
}%

\BiblioItem{texVectorSpace}{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{texVectorSpace}{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

%\BiblioItem{texVectorSpace}{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{texVectorSpace}{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{texReferenceFrame}{math.DG-0412391}
{
Александр Клейн,
Frame Manifold,
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2004)
}%

\BiblioItem{texAlgebraBundle,texBundleRelation}{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2007)
}%

\BiblioItem{texBundleRelation,texPrefaceRelation}{0702.561}
{
Александр Клейн,
Расслоенная алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

%\BiblioItem{texBasis,texLinearMap}{math.RA-0501237}
%{
%Александр Клейн,
%Векторное пространство над телом,\\
%eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2005)
%}%

\BiblioItem{texPolymodule}{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Skew-Field, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\ifx\PrintBook\Defined
\else
\BiblioItem{texVectorSpace,texAlgebraBundle}{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2006)
}%
\fi

\BiblioItem{texHomotopy}{q-alg-9705009}
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{texIntro}{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81 (1967)
}%

\BiblioItem{texPrefaceRelation}{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem{texBundleRelation,texPrefaceRelation}{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem{texAlgebraBundle}{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{texBundleRelation}{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{texCalculus}{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem{texCalculus}{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{texCalculus}{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология, Использование вещественных чисел в общей топологии,
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
М. Наука, 1975
}

\BiblioItem{texAlgebraBundle}{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\CloseBiblio



==> CommandsRussian.tex <==
%auto-ignore
%\usepackage{cmap}
%\usepackage{cmcyralt}
%\usepackage{cmcyr}
%\usepackage{lhcyr}
%\usepackage{cmlgc}
\def\UseRussian{}
\usepackage[T2A,T2B]{fontenc}
\usepackage[cp1251]{inputenc}
\usepackage[english,russian]{babel}
\selectlanguage{russian}


==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index{texLinearMap}%1%1
   {$1$-\drc форма}%
   {1-drc form, vector spaces}%
\SetIndexSpace%
\Index{texPolymodule}%2%66
   {$(2)$\hyph векторное пространство}%
   {(2)-vector space}%
\Index{texBundleRelation}%2%122
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index{texBiring}%A%2
   {$(^{\gi a}_{\gi b})$\hyph \CR квазидетерминант}%
   {a b cr-quasideterminant}%
\Index{texBiring}%A%34
   {$(^{\gi a}_{\gi b})$\hyph \RC квазидетерминант}%
   {a b RC-quasideterminant}%
\Index{texCalculus}%A%67
   {$A$\Hyph значная функция}%
   {A valued function}%
\SetIndexSpace%
\Index{texBiring}%C%3
   {\subs строка матрицы}%
   {c row}%
\Index{texHomotopy}%C%4
   {Category of \drc vector spaces}%
   {Category of Drc vector spaces}%
\Index{texVectorSpace}%C%5
   {\CR матричная группа}%
   {cr-matrix group}%
\Index{texBiring}%C%6
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index{texBiring}%C%7
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index{texBiring}%C%8
   {\CR степень}%
   {cr power}%
\Index{texVectorSpace}%C%9
   {\crd векторное пространство}%
   {crd vector space}%
\Index{texBiring}%C%10
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index{texVectorSpace}%D%11
   {\dcr базис векторного пространства \subs строк}%
   {dcr basis, c rows vector space}%
\Index{texVectorSpace}%D%12
   {\dcr вектор}%
   {dcr vector}%
\Index{texVectorSpace}%D%13
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index{texVectorSpace}%D%14
   {\dcr векторное пространство \subs строк}%
   {subs rows dcr vector space}%
\Index{texVectorSpace}%D%15
   {\drc  линейно зависимые векторы}%
   {linearly dependent, vector space}%
\Index{texVectorSpace}%D%55
   {\drc автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index{texVectorSpace}%D%17
   {\drc базис}%
   {}%
\SubIndex{texVectorSpace}%4%
   {в векторном пространстве}%
   {drc basis, vector space}%
\SubIndex{texVectorSpace}%5%
   {в векторном пространстве \sups строк}%
   {drc basis, r rows vector space}%
\Index{texVectorSpace}%D%18
   {\drc вектор}%
   {drc vector}%
\Index{texVectorSpace}%D%19
   {\drc векторное пространство}%
   {drc vector space}%
\Index{texVectorSpace}%D%20
   {\drc векторное пространство \sups строк}%
   {sups rows drc vector space}%
\Index{texCalculus}%D%46
   {\drc вектор\hyph функция}%
   {drc vector function}%
\Index{texVectorSpace}%D%83
   {\drc изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index{texVectorSpace}%D%87
   {drc координатное векторное пространство}%
   {drc coordinate vector space}%
\Index{texVectorSpace}%D%23
   {\drc линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Index{texReferenceFrame}%D%24
   {\drc линейно независимыe векторы}%
   {linearly independent vector fields}%
\Index{texVectorSpace}%D%114
   {\drc линейно независимые векторы}%
   {linearly independent, vector space}%
\Index{texVectorSpace}%D%25
   {\drc линейное отображение векторных пространств}%
   {drc linear map of vector spaces}%
\Index{texVectorSpace}%D%27
   {$D\star$\hyph векторное пространство}%
   {Dstar vector space}%
\Index{texVectorSpace}%D%26
   {$D\star$\hyph произведение вектора на скаляр}%
   {Dstar product of vector over scalar, vector space}%
\Index{texCalculus}%D%96
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\SetIndexSpace%
\Index{texELie}%E%28
   {enhanced Lie group}%
   {enhanced Lie group}%
\Index{texDiffEq}%E%29
   {essential parameters}%
   {essential parameters}%
\SetIndexSpace%
\Index{texTypeBasis}%G%30
   {\Gbasis}%
   {G-basis}%
\Index{texTypeBasis}%G%31
   {\Gcoords ы}%
   {G-coordinates}%
\Index{texTypeBasis}%G%32
   {\Gspace о}%
   {GSpace}%
\Index{texBasis}%G%267
   {\Gbasis\ векторного пространства}%
   {G-basis}%
\Index{texBasis}%G%270
   {\Gcoords ы базиса}%
   {G-coordinates}%
\Index{texBasis}%G%271
   {\Gspace о}%
   {GSpace}%
\SetIndexSpace%
\Index{texPolymodule}%N%231
   {$(n)$\hyph векторное пространство}%
   {(n)-vector space}%
\Index{texBundleRelation}%N%218
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index{texBiring}%R%35
   {\sups строка матрицы}%
   {r row}%
\Index{texVectorSpace}%R%36
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index{texVectorSpace}%R%37
   {\RC главный минор}%
   {RC-major minor}%
\Index{texBiring}%R%38
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index{texVectorSpace}%R%39
   {\RC матричная группа}%
   {rc-matrix group}%
\Index{texVectorSpace}%R%40
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index{texBiring}%R%41
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index{texBiring}%R%42
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index{texVectorSpace}%R%43
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index{texBiring}%R%44
   {\RC степень}%
   {rc power}%
\Index{texVectorSpace}%R%45
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index{texVectorSpace}%R%213
   {$R\star$\Hyph модуль}%
   {Rstar-module}%
\Index{texBiring}%R%47
   {$r$\hyph строка матрицы}%
   {r-row}%
\SetIndexSpace%
\Index{texLinearMap}%S%48
   {$\star D$\Hyph произведением \drc линейного отображения $A$ на скаляр}%
   {starD product of drc linear map over scalar}%
\Index{texVectorSpace}%S%217
   {$\star D$\hyph векторное пространство}%
   {starD-vector space}%
\Index{texVectorSpace}%S%216
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index{texDrcRepresentation}%S%49
   {\sT сдвиг}%
   {starT shift}%
\Index{texAlgebraBundle}%S%50
   {\sT сдвиг на расслоении групп}%
   {starT shift, group bundle}%
\SetIndexSpace%
\Index{texVectorSpace}%T%51
   {\Ts векторное пространство матриц}%
   {matrices vector space}%
\Index{texVectorSpace}%T%52
   {\Ts линейная комбинация векторов}%
   {linear composition of  vectors}%
\Index{texDrcRepresentation}%T%53
   {\Ts сдвиг}%
   {Tstar shift}%
\SetIndexSpace%
\Index{texNewton}%V%54
   {vector potential}%
   {vector potential}%
\SetIndexSpace%
\Index{texAffine}%А%56
   {автопараллельная кривая}%
   {auto parallel line}%
\Index{texDrcBasis}%А%57
   {активное \sT представление}%
   {active representation, vector space}%
\Index{texBasis}%А%262
   {активное представление}%
   {active representation}%
\Index{texBasis}%А%263
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index{texLie}%А%58
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\SubIndex{texLie}%9%
   {определённая слева}%
   {left defined algebra Lie}%
\SubIndex{texLie}%10%
   {определённая справа}%
   {right defined algebra Lie}%
\Index{texBiring}%А%59
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index{texAlgebraBundle}%А%60
   {антигомоморфизм расслоенных групп}%
   {antihomomorphism of group bundles}%
\Index{texBundleRelation}%А%156
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index{texAlgebraBundle}%А%61
   {арность операции}%
   {arity of operation}%
\Index{texBasis}%А%277
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index{texBasis}%А%275
   {аффинный базис}%
   {Affine Basis}%
\SetIndexSpace%
\Index{texAlgebraBundle}%Б%172
   {база отображения}%
   {base of map}%
\Index{texBundleRelation}%Б%233
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index{texTypeBasis}%Б%16
   {базис}%
   {}%
\SubIndex{texTypeBasis}%1%
   {аффинный}%
   {Affine Basis}%
\SubIndex{texTypeBasis}%2%
   {ортонормальный}%
   {Orthonornal Basis}%
\SubIndex{texTypeBasis}%3%
   {центро-аффинный}%
   {Central Affine Basis}%
\Index{texBasis}%Б%266
   {базис векторного пространства}%
   {Basis}%
\Index{texLieRepresentation}%Б%62
   {базовый вектор}%
   {}%
\SubIndex{texLieRepresentation}%11%
   {\sT представления}%
   {basis vector of starT representation}%
\SubIndex{texLieRepresentation}%12%
   {\Ts представления}%
   {basis vector of Tstar representation}%
\Index{texLie}%Б%63
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index{texLieRepresentation}%Б%64
   {бесконечно малый генератор}%
   {infinitesimal generator}%
\Index{texBiring}%Б%65
   {бикольцо}%
   {biring}%
\SetIndexSpace%
\Index{texPolymodule}%В%230
   {($D_1\RCstar$, ..., $D_n\RCstar$)\hyph векторное пространство}%
   {(d1rc,dnrc)-vector space}%
\Index{texPolymodule}%В%229
   {($S\star$, $\star T$)\hyph векторное пространство}%
   {(Sstar,starT)-vector space}%
\Index{texDiffProperty}%В%69
   {вектор Килинга второго рода}%
   {Killing vector second type}%
\Index{texRepresentation}%В%261
   {вектор\hyph столбец}%
   {column vector}%
\Index{texAlgebraBundle}%В%70
   {векторное расслоение}%
   {vector bundle}%
\Index{texRepresentation}%В%260
   {вектор\hyph строка}%
   {row vector}%
\Index{texDiffEq}%В%71
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index{texNewton}%В%72
   {второй закон Ньютона}%
   {Second Newton law}%
\SetIndexSpace%
\Index{texBasis}%Г%264
   {группа симметрии}%
   {symmetry group}%
\Index{texDrcBasis}%Г%73
   {геометрический объект}%
   {}%
\SubIndex{texDrcBasis}%13%
   {в координатном представлении,	определённом в векторном пространстве}%
   {geometrical object, coordinate vector space}%
\SubIndex{texDrcBasis}%14%
   {определённый в векторном пространстве}%
   {geometrical object, vector space}%
\SubIndex{texDrcBasis}%15%
   {типа $A$}%
   {geometrical object of type A, vector space}%
\Index{texBasis}%Г%290
   {геометрический объект в векторном пространстве}%
   {geometrical object, vector space}%
\Index{texBasis}%Г%288
   {геометрический объект в координатном представлении}%
   {geometrical object, coordinate vector space}%
\Index{texBasis}%Г%293
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometrical object of type A, vector space}%
\Index{texReferenceFrame}%Г%74
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index{texAlgebraBundle}%Г%75
   {гомоморфизм расслоенных алгебр}%
   {homomorphism of algebra bundles}%
\Index{texAlgebraBundle}%Г%76
   {гомоморфизм расслоенных групп}%
   {homomorphism of group bundles}%
\Index{texTypeBasis}%Г%77
   {группа аффинных преобразований}%
   {AffineTransformationGroup}%
\Index{texBasis}%Г%274
   {группа аффинных преобразований}%
   {AffineTransformationGroup}%
\Index{texDrcBasis}%Г%78
   {группа симметрии}%
   {SymmetryGroup}%
\Index{texGroupRing}%Г%79
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index{}%Д%283
   {движение на многообразии базисов}%
   {movement transformation}%
\Index{texAlgebraBundle}%Д%176
   {декартова степень расслоения}%
   {Cartesian power of bundle}%
\Index{texAlgebraBundle}%Д%180
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index{texAlgebraBundle}%Д%181
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index{texBundleRelation}%Д%227
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index{texCalculus}%Д%105
   {дифференциал отображения нормированного \drc векторного пространства в нормированное тело}%
   {differential, drc vector space to skew field}%
\Index{texCalculus}%Д%99
   {дифференцируемая функция \drc векторного пространства в тело $D$ }%
   {differentiable functions, drc vector space to skew field}%
\Index{texBundleRelation}%Д%113
   {иагональ в расслоении}%
   {diagonal in bundle}%
\SetIndexSpace%
\Index{texDrcRepresentation,texLinearMap,texVectorSpace}%З%80
   {закон ассоциативности}%
   {}%
\SubIndex{texVectorSpace}%17%
   {для \drc линейных отображений векторных пространств}%
   {associative law for drc linear maps of vector spaces}%
\SubIndex{texVectorSpace}%16%
   {для \Ts векторного пространства}%
   {associative law, Tstar vector space}%
\SubIndex{texDrcRepresentation}%18%
   {для ковариантного \Ts представления}%
   {associative law for Tstar covariant representation}%
\SubIndex{texLinearMap}%19%
   {для парных представлений}%
   {associative law for twin representations}%
\Index{texBundleRelation}%З%155
   {закон ассоциативности произведения расслоенных соответствий}%
   {associative law, composition of fibered correspondences}%
\Index{texVectorSpace}%З%81
   {закон дистрибутивности}%
   {}%
\SubIndex{texVectorSpace}%20%
   {\Ts векторное пространство}%
   {distributive law, Tstar vector space}%
\Index{texVectorSpace}%З%82
   {закон унитарности}%
   {}%
\SubIndex{texVectorSpace}%21%
   {для \Ts векторного пространства}%
   {unitarity law, Tstar vector space}%
\SetIndexSpace%
\Index{texAlgebraBundle}%И%84
   {изоморфизм расслоенных алгебр}%
   {isomorphism of algebra bundles}%
\Index{texLinearLie}%И%85
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index{texBundleRelation}%К%111
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index{texBundleRelation}%К%112
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index{texBasis}%К%278
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index{texBasis}%К%284
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index{texBundleRelation}%К%228
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index{texVectorSpace}%К%21
   {координатная матрица}%
   {}%
\SubIndex{texVectorSpace}%6%
   {вектора в \drc базисе}%
   {coordinate matrix of vector in drc basis}%
\SubIndex{texVectorSpace}%7%
   {множества векторов в векторном пространстве \dcr строк}%
   {coordinate matrix of set of vectors, dcr vector space}%
\SubIndex{texVectorSpace}%8%
   {множества векторов в векторном пространстве \drc строк}%
   {coordinate matrix of set of vectors, drc vector space}%
\Index{texReferenceFrame}%К%86
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index{texGenRelativity}%К%239
   {координатная система отсчёта в пространстве событий}%
   {coordinate reference frame in event space}%
\Index{texBasis}%К%285
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index{texDrcBasis}%К%88
   {координатное представление в \drc векторном пространстве}%
   {coordinate representation, vector space}%
\Index{texBasis}%К%287
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index{texBasis}%К%286
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index{texVectorSpace}%К%89
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index{texVectorSpace}%К%22
   {координаты вектора в \drc базисе}%
   {coordinates of vector in drc basis}%
\Index{texDrcBasis}%К%90
   {координаты геометрического объекта}%
   {}%
\SubIndex{texDrcBasis}%22%
   {в векторном пространстве}%
   {coordinates of geometrical object, vector space}%
\SubIndex{texDrcBasis}%23%
   {в координатном векторном пространстве}%
   {coordinates of geometrical object, coordinate vector space}%
\Index{texBasis}%К%291
   {координаты геометрического объекта}%
   {coordinates of geometrical object, vector space}%
\Index{texBasis}%К%289
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometrical object, coordinate vector space}%
\Index{texVectorSpace}%К%91
   {координаты множества векторов в \dcr векторном пространстве}%
   {coordinates of set of vectors, dcr vector space}%
\Index{texVectorSpace}%К%92
   {координаты множества векторов в \drc векторном пространстве}%
   {coordinates of set of vectors, drc vector space}%
\Index{texDrcBasis}%К%93
   {координаты представления}%
   {coordinates of representation}%
\Index{texBasis}%К%265
   {координаты представления}%
   {coordinates of representation}%
\Index{texAffine}%К%94
   {кривизна Картана}%
   {Cartan curvature}%
\Index{texAffine}%К%95
   {кручение}%
   {torsion}%
\SetIndexSpace%
\Index{texVectorSpace}%Л%98
   {левое векторное пространство}%
   {left vector space}%
\Index{texLie}%Л%101
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index{texRepresentation}%Л%247
   {левостороннее ковариантное представление группы}%
   {left-side covariant representation}%
\Index{texRepresentation}%Л%249
   {левостороннее контравариантное представление группы}%
   {left-side contravariant representation}%
\Index{texRepresentation}%Л%244
   {левостороннее представление группы}%
   {left-side representation of group}%
\Index{texRepresentation}%Л%242
   {левостороннее преобразование}%
   {left-side transformation}%
\Index{texLie}%Л%103
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index{texVectorSpace}%Л%214
   {левый модуль}%
   {left module}%
\Index{texDrcRepresentation}%Л%108
   {левый сдвиг}%
   {left shift}%
\Index{texRepresentation}%Л%251
   {левый сдвиг на группе}%
   {left shift, group}%
\Index{texAlgebraBundle}%Л%109
   {левый сдвиг на расслоении групп}%
   {Tstar shift, group bundle}%
\Index{texReferenceFrame}%Л%110
   {линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index{texRepresentation}%Л%240
   {линейное представление группы}%
   {linear representation of group}%
\Index{texAlgebraBundle}%Л%116
   {лифт отображения}%
   {lift of map}%
\Index{texBundleRelation}%Л%232
   {лифт соответствия}%
   {lift of correspondence}%
\Index{texReferenceFrame}%Л%117
   {локальная система отсчёта}%
   {local reference frame}%
\SetIndexSpace%
\Index{texVectorSpace}%М%118
   {матрица \drc линейное отображениеа}%
   {matrix of drc linear map}%
\Index{texAffine}%М%119
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index{texDrcBasis}%М%120
   {многообразие базисов}%
   {}%
\SubIndex{texDrcBasis}%24%
   {\drc векторного пространства}%
   {basis manifold of vector space}%
\SubIndex{texTypeBasis}%25%
   {аффинного пространства}%
   {Basis Manifold, Affine Space}%
\SubIndex{texTypeBasis}%26%
   {евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\SubIndex{texTypeBasis}%27%
   {центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index{texBasis}%М%276
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index{texBasis}%М%268
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index{texBasis}%М%282
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index{texBasis}%М%280
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index{texReferenceFrame}%М%123
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\SetIndexSpace%
\Index{texVectorSpace}%Н%124
   {невырожденная система \drc линейных уравнений}%
   {nonsingular system of linear equations}%
\Index{texRepresentation}%Н%241
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index{texReferenceFrame}%Н%125
   {неголономная координата}%
   {anholonomic coordinate}%
\Index{texReferenceFrame}%Н%126
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index{texReferenceFrame}%Н%127
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index{texAffine}%Н%128
   {неметричность}%
   {nonmetricity}%
\Index{texCalculus}%Н%97
   {норма на \drc векторном пространстве}%
   {norm on drc vector space}%
\Index{texCalculus}%Н%100
   {норма на теле}%
   {absolute value on skew field}%
\Index{texCalculus}%Н%102
   {нормированное тело}%
   {valued skew field}%
\Index{texCalculus}%Н%104
   {нормированным \drc векторное пространство}%
   {normed drc vector space}%
\SetIndexSpace%
\Index{texBundleRelation}%О%121
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index{texBundleRelation}%О%115
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index{texBiring}%О%129
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index{texReferenceFrame}%О%130
   {объект неголономности}%
   {anholonomity object}%
\Index{texDrcRepresentation}%О%131
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index{texRepresentation}%О%259
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index{texAlgebraBundle}%О%132
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of group bundle}%
\Index{texRepresentation}%О%258
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index{texAlgebraBundle}%О%133
   {операция на расслоении}%
   {operation on bundle}%
\Index{texBiring}%О%134
   {определитель матрицы}%
   {determinant}%
\Index{texDrcRepresentation}%О%135
   {орбита \Ts представления группы}%
   {orbit of representation of group}%
\Index{texRepresentation}%О%253
   {орбита представления группы}%
   {orbit of representation of group}%
\Index{texAlgebraBundle}%О%136
   {орбита представления расслоенной группы}%
   {orbit of representation of group bundle}%
\Index{texBasis}%О%281
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Index{texTidal}%О%137
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index{texReferenceFrame}%О%138
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\SetIndexSpace%
\Index{texReferenceFrame}%П%139
   {параллелограм}%
   {parallelogram}%
\Index{texAlgebraBundle,texDrcRepresentation,texLinearMap}%П%140
   {парные преставления}%
   {}%
\SubIndex{texDrcRepresentation}%28%
   {группы}%
   {twin representations of group}%
\SubIndex{texAlgebraBundle}%29%
   {расслоенной группы}%
   {twin representations of group bundle}%
\SubIndex{texLinearMap}%30%
   {тела}%
   {twin representations of skew field}%
\Index{texDrcBasis}%П%141
   {пассивное \Ts представление}%
   {passive representation}%
\Index{texBasis}%П%273
   {пассивное представление}%
   {passive representation}%
\Index{texBasis}%П%272
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index{texNewton}%П%142
   {первый закон Ньютона}%
   {First Newton law}%
\Index{texAffine}%П%143
   {перенос Картана}%
   {Cartan transport}%
\Index{texAffine}%П%144
   {перенос Френе}%
   {Frenet transport}%
\Index{texBundleRelation}%П%220
   {подрасслоение}%
   {subbundle}%
\Index{texNewton}%П%146
   {потенциальная энергия}%
   {potential energy}%
\Index{texVectorSpace}%П%149
   {правое векторное пространство}%
   {right vector space}%
\Index{texLie}%П%151
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index{texRepresentation}%П%248
   {правостороннее ковариантное представление группы}%
   {right-side covariant representation}%
\Index{texRepresentation}%П%250
   {правостороннее контравариантное представление группы}%
   {right-side contravariant representation}%
\Index{texRepresentation}%П%245
   {правостороннее представление группы}%
   {right-side representation of group}%
\Index{texRepresentation}%П%243
   {правостороннее преобразование}%
   {right-side transformation}%
\Index{texLie}%П%153
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index{texVectorSpace}%П%215
   {правый модуль}%
   {right module}%
\Index{texDrcRepresentation}%П%158
   {правый сдвиг}%
   {right shift}%
\Index{texRepresentation}%П%252
   {правый сдвиг на группе}%
   {right shift, group}%
\Index{texBasis}%П%292
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometrical object, vector space}%
\Index{texDrcBasis}%П%159
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometrical object, vector space}%
\Index{texDrcRepresentation}%П%160
   {представление алгебры $A$}%
   {}%
\SubIndex{texDrcRepresentation}%31%
   {\sT}%
   {starT representation of algebra}%
\SubIndex{texDrcRepresentation}%32%
   {\Ts}%
   {Tstar representation of algebra}%
\SubIndex{texDrcRepresentation}%33%
   {левостороннее}%
   {left-side representation of algebra}%
\SubIndex{texDrcRepresentation}%34%
   {однотранзитивное}%
   {single transitive representation of algebra}%
\SubIndex{texDrcRepresentation}%35%
   {правостороннее}%
   {right-side representation of algebra}%
\SubIndex{texDrcRepresentation}%36%
   {транзитивное}%
   {transitive representation of algebra}%
\SubIndex{texDrcRepresentation}%37%
   {эффективное}%
   {effective representation of algebra}%
\Index{texDrcRepresentation}%П%161
   {представление группы}%
   {}%
\SubIndex{texDrcBasis}%38%
   {\drc линейное \sT}%
   {linear representation of group}%
\SubIndex{texDrcBasis}%39%
   {\rcd}%
   {rcd linear representation of group}%
\SubIndex{texDrcRepresentation}%40%
   {\sT}%
   {starT representation of group}%
\SubIndex{texDrcRepresentation}%41%
   {\Ts}%
   {Tstar representation of group}%
\SubIndex{texDrcRepresentation}%42%
   {ковариантное \Ts}%
   {Tstar covariant representation of group}%
\SubIndex{texDrcRepresentation}%43%
   {контравариантное \Ts}%
   {Tstar contravariant representation of group}%
\SubIndex{texDrcRepresentation}%44%
   {эффективное}%
   {effective representation of group}%
\Index{texRepresentation}%П%246
   {представление группы}%
   {representation of group}%
\Index{texAlgebraBundle}%П%162
   {представление расслоенной алгебры}%
   {}%
\SubIndex{texAlgebraBundle}%45%
   {\sT}%
   {starT representation of algebra bundle}%
\SubIndex{texAlgebraBundle}%46%
   {\Ts}%
   {Tstar representation of algebra bundle}%
\SubIndex{texAlgebraBundle}%47%
   {левостороннее}%
   {left-side representation of algebra bundle}%
\SubIndex{texAlgebraBundle}%48%
   {однотранзитивное}%
   {single transitive representation of algebra bundle}%
\SubIndex{texAlgebraBundle}%49%
   {правостороннее}%
   {right-side representation of algebra bundle}%
\SubIndex{texAlgebraBundle}%50%
   {транзитивное}%
   {transitive representation of algebra bundle}%
\SubIndex{texAlgebraBundle}%51%
   {эффективное}%
   {effective representation of algebra bundle}%
\Index{texAlgebraBundle}%П%163
   {представление расслоенной группы}%
   {}%
\SubIndex{texAlgebraBundle}%52%
   {\sT}%
   {starT representation of group bundle}%
\SubIndex{texAlgebraBundle}%53%
   {\Ts}%
   {Tstar representation of group bundle}%
\SubIndex{texAlgebraBundle}%54%
   {\Ts ковариантное}%
   {Tstar covariant representation of group bundle}%
\SubIndex{texAlgebraBundle}%55%
   {\Ts контравариантное}%
   {Tstar contravariant representation of group bundle}%
\SubIndex{texAlgebraBundle}%56%
   {эффективное}%
   {effective representation of group bundle}%
\Index{texDrcRepresentation}%П%164
   {преобразование}%
   {}%
\SubIndex{texDrcRepresentation}%57%
   {\sT}%
   {starT transformation}%
\SubIndex{texDrcRepresentation}%58%
   {\Ts}%
   {Tstar transformation}%
\SubIndex{texDrcRepresentation}%59%
   {левостороннее}%
   {left-side transformation}%
\SubIndex{texDrcRepresentation}%60%
   {невырожденное}%
   {nonsingular transformation}%
\SubIndex{texDrcRepresentation}%61%
   {правостороннее}%
   {right-side transformation}%
\Index{texGenRelativity}%П%165
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index{texDrcBasis}%П%166
   {преобразование на многообразии базисов}%
   {}%
\SubIndex{texDrcBasis}%62%
   {активное}%
   {active transformation, vector space}%
\SubIndex{texTypeBasis}%63%
   {аффинное}%
   {affine transformation}%
\SubIndex{texTypeBasis}%64%
   {движение}%
   {movement transformation}%
\SubIndex{texTypeBasis}%65%
   {квазиаффинное}%
   {quasi affine transformation}%
\SubIndex{texTypeBasis}%66%
   {квазидвижение}%
   {quasi movement}%
\SubIndex{texDrcBasis}%67%
   {пассивное}%
   {passive transformation, vector space}%
\Index{texAlgebraBundle}%П%167
   {преобразование расслоения}%
   {}%
\SubIndex{texAlgebraBundle}%68%
   {\sT}%
   {starT transformation of bundle}%
\SubIndex{texAlgebraBundle}%69%
   {\Ts}%
   {Tstar transformation of bundle}%
\SubIndex{texAlgebraBundle}%70%
   {левостороннее}%
   {left-side transformation of bundle}%
\SubIndex{texAlgebraBundle}%71%
   {невырожденное}%
   {nonsingular transformation of bundle}%
\Index{texAlgebraBundle}%П%221
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index{texAlgebraBundle}%П%222
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index{texBundleRelation,texBundleRelation}%П%225
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {reduced fibered correspondence from A to B}%
\Index{texBundleRelation}%П%226
   {приведенное расслоенное соответствие в $\mathcal{A}$}%
   {reduced fibered correspondence in A}%
\Index{texBiring}%П%168
   {приводимое бикольцо}%
   {reducible biring}%
\Index{texBiring}%П%169
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index{texBiring}%П%170
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index{texDrcBasis}%П%171
   {принцип инвариантности}%
   {invariance principle}%
\Index{texBasis}%П%296
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index{texBundleRelation}%П%235
   {продолжение соответствия}%
   {extension of correspondence}%
\Index{texDrcBasis}%П%173
   {произведение геометрического объекта и константы}%
   {product of geometrical object and constant}%
\Index{texBasis}%П%295
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometrical object and constant, vector space}%
\Index{texBundleRelation}%П%154
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index{texBundleRelation}%П%188
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\SubIndex{texVectorSpace}%74%
   {\drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\SubIndex{texVectorSpace}%75%
   {\rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index{texAffine}%П%174
   {производная Картана}%
   {Cartan derivative}%
\Index{texDiffProperty}%П%175
   {производная Ли}%
   {Lie derivative}%
\SubIndex{texDiffProperty}%72%
   {метрики}%
   {Lie derivative of metric}%
\SubIndex{texDiffProperty}%73%
   {связности}%
   {Lie derivative of connection}%
\Index{texBundleRelation}%П%236
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index{texLieRepresentation}%П%177
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index{texDrcRepresentation}%П%178
   {прямое произведение \Ts представлений группы}%
   {direct product of representations of group}%
\Index{texRepresentation}%П%254
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index{texAlgebraBundle}%П%179
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of group bundle}%
\Index{texReferenceFrame}%П%182
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index{texVectorSpace}%Р%183
   {размерность \drc векторного пространства}%
   {dimension of vector space}%
\Index{texAlgebraBundle}%Р%184
   {расслоенная алгебра}%
   {algebra bundle}%
\Index{texAlgebraBundle}%Р%185
   {расслоенная группа}%
   {group bundle}%
\Index{texAlgebraBundle}%Р%186
   {расслоенная подалгебра}%
   {subalgebra bundle}%
\Index{texBundleRelation}%Р%145
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index{texBundleRelation}%Р%237
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index{texBundleRelation}%Р%238
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index{texAlgebraBundle}%Р%187
   {расслоенное кольцо}%
   {ring bundle}%
\Index{texBundleRelation}%Р%219
   {расслоенное подмножество}%
   {fibered subset}%
\Index{texBundleRelation}%Р%224
   {расслоенное соответствие в $\mathcal{A}$}%
   {fibered correspondence in A}%
\Index{texBundleRelation}%Р%223
   {расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered correspondence from A to B}%
\Index{texBundleRelation}%Р%157
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\SetIndexSpace%
\Index{texAffine}%С%189
   {связность Картана}%
   {Cartan connection}%
\Index{texAffine}%С%190
   {символ Картана}%
   {Cartan symbol}%
\Index{texBiring}%С%191
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index{texBundleRelation}%С%148
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index{texGenRelativity}%С%192
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index{texVectorSpace}%С%193
   {система \drc линейных уравнений}%
   {system of linear equations}%
\Index{texGenRelativity}%С%194
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index{texReferenceFrame}%С%195
   {система отсчёта на многообразии}%
   {reference frame}%
\Index{texNewton}%С%196
   {скалярный потенциал}%
   {scalar potential}%
\Index{texTidal}%С%197
   {скорость отклонения}%
   {speed of deviation}%
\Index{texBiring}%С%198
   {стандартное представление матрицы}%
   {Standard representation}%
\Index{texDrcBasis}%С%199
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index{texBasis}%С%269
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index{texBundleRelation}%С%234
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index{texLinearMap}%С%200
   {сумма \drc линейных отображений}%
   {sum of drc linear maps, drc vector spaces}%
\Index{texDrcBasis}%С%201
   {сумма геометрических объектов}%
   {sum of geometrical objects}%
\Index{texBasis}%С%294
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometrical objects, vector space}%
\SetIndexSpace%
\Index{texNewton}%Т%202
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index{texLie}%Т%203
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index{texVectorSpace}%Т%204
   {тип векторного пространства}%
   {vector space type}%
\Index{texReferenceFrame}%Т%205
   {типа $G$ система отсчёта}%
   {type G reference frame}%
\Index{texCalculus}%Т%152
   {топологическое \drc векторное пространство}%
   {topological drc vector space}%
\Index{texCalculus}%Т%33
   {топологическое тело}%
   {topological skew field}%
\Index{texBundleRelation}%Т%147
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index{texRepresentation}%Т%257
   {транзитивное представление группы}%
   {transitive representation of group}%
\SetIndexSpace%
\Index{texDiffProperty}%У%206
   {уравнение Килинга}%
   {Killing equation}%
\Index{texDiffProperty}%У%207
   {уравнение Килинга второго рода}%
   {Killing equation second type}%
\Index{texBiring}%У%208
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index{texCalculus}%Ф%150
   {функция $\gi n$ $D$\Hyph значных переменных}%
   {function of n D valued variables}%
\Index{texCalculus}%Ф%68
   {функция, непрерывная по совокупности аргументов}%
   {function continuous with respect to set of arguments}%
\SetIndexSpace%
\Index{texBasis}%Ц%279
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index{texCalculus}%Ч%106
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping with respect to variable, skew field}%
\Index{texCalculus}%Ч%107
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping with respect to variable, drc vector space}%
\SetIndexSpace%
\Index{texAffine}%Э%209
   {экстремальная кривая}%
   {extreme line}%
\Index{texRepresentation}%Э%256
   {эффективное представление группы}%
   {effective representation of group}%
\Index{texVectorSpace}%Э%210
   {эффективное представление тела}%
   {effective representation of skew field}%
\SetIndexSpace%
\Index{texDrcRepresentation}%Я%211
   {ядро неэффективности \Ts представления группы $G$}%
   {kernel of inefficiency of representation of group}%
\Index{texRepresentation}%Я%255
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index{texAlgebraBundle}%Я%212
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of group bundle}%

\CloseIndex


==> Representation.Russian.tex <==
%auto-ignore
\def\texRepresentation{}
\ifx\PrintBook\undefined

\section{Введение}

Эта статья была написана под большим влиянием книги \citeBib{Rashevsky}.
Изучение однородного пространства группы симметрий векторного пространства
ведёт нас к определению базиса этого пространства
и многообразия базисов.
Мы вводим два типа преобразований многообразия базисов:
активные и пассивные преобразования. Различие между ними состоит в том,
что активное преобразование может быть выражено как преобразование
исходного пространства.
Как показано в \citeBib{Rashevsky}, пассивное преобразование
даёт возможность определить
понятия инвариантности и геометрического объекта.

Мы имеем
две противоположные точки зрения на геометрический объект.
С одной стороны мы фиксируем координаты геометрического объекта
относительно заданного базиса и указываем закон преобразования
координат при замене базиса. В то же время мы рассматриваем
всю совокупность координат геометрического объекта
относительно различных базисов как единое целое. Это
даёт нам возможность бескоординатного
изучения геометрического объекта.
\else
				\chapter{Представление группы}
				\label{chapter: Representation of Group}
\fi
			\section{Представление}

	\begin{definition}
	\label{definition: nonsingular transformation} 
Мы будем называть отображение
\[
t:M\rightarrow M
\]
\AddIndex{невырожденным преобразованием}{nonsingular transformation},
если существует обратное отображение.
	 \qed
	 \end{definition}

	 \begin{definition}
Преобразование называется
\AddIndex{левосторонним преобразованием}{left-side transformation}
если оно действует слева
\[
u'=t u
\]
Мы будем обозначать
\symb{l(M)}1{set of left-side nonsingular transformations}
множество левосторонних невырожденных преобразований множества $M$.
	 \qed
	 \end{definition}

	 \begin{definition}
Преобразование называется
\AddIndex{правосторонним преобразованием}{right-side transformation}
если оно действует справа
\[
u'= ut
\]
Мы будем обозначать
\symb{r(M)}1{set of right-side nonsingular transformations}
множество правосторонних невырожденных преобразований множества $M$.
	 \qed
	 \end{definition}

Мы будем обозначать
\symb{\delta}1{identical transformation}
тождественное преобразование.

		\begin{definition}
		\label{definition: left-side representation of group} 
Пусть $G$ - группа.
Мы будем называть отображение
	\begin{equation}
f:G\rightarrow l(M)
	\label{eq: left-side representation of group}
	\end{equation}
\AddIndex{левосторонним представлением группы}
{left-side representation of group}
$G$ в множестве $M$, если отображение $f$ удовлетворяет условиям
	\begin{equation}
f(ab)u=f(a)(f(b)u)
	\label{eq: left-side product of transformations}
	\end{equation}
	\begin{equation}
f(e)=\delta
	\label{eq: left-side identical transformation}
	\end{equation}
		\qed
		\end{definition}

		\begin{definition}
		\label{definition: right-side representation of group} 
Пусть $G$ - группа.
Мы будем называть отображение
	\begin{equation}
f:G\rightarrow r(M)
	\label{eq: right-side representation of group}
	\end{equation}
\AddIndex{правосторонним представлением группы}
{right-side representation of group}
$G$ в множестве $M$, если отображение $f$ удовлетворяет условиям
	\begin{equation}
uf(ab)=(uf(a))f(b)
	\label{eq: right-side product of transformations}
	\end{equation}
	\begin{equation}
f(e)=\delta
	\label{eq: right-side identical transformation}
	\end{equation}
		\qed
		\end{definition}

Любое утверждение, справедливое для
левостороннего представления группы,
будет справедливо для правостороннего представления.
Поэтому мы будем пользоваться общим термином
\AddIndex{представление группы}{representation of group}
и будем пользоваться обозначениями для левостороннего
представления в тех случаях, когда это не вызывает
недоразумения.

			\begin{theorem}
			\label{theorem: inverse transformation}
Для любого $g\in G$
	\begin{equation}
	\label{eq: inverse transformation}
f(g^{-1})=f(g)^{-1}
	\end{equation}
		\end{theorem}
		\begin{proof}
На основании \eqref{eq: left-side product of transformations}
и \eqref{eq: left-side identical transformation},
мы можем записать
\[
u=\delta u=f(gg^{-1})u=f(g)(f(g^{-1})u)
\]
Это завершает доказательство.
		\end{proof}

		\begin{theorem}
		\label{theorem: left-side covariant representation}
Пусть $l(M)$ - группа относительно умножения
	\begin{equation}
(t_1t_2)u=t_1(t_2u)
	\label{eq: left-side covariant product of transformations}
	\end{equation}
и $\delta$ - единица группы $l(M)$.
Если отображение
\eqref{eq: left-side representation of group}
является гомоморфизмом групп
	\begin{equation}
f(ab)=f(a)f(b)
	\label{eq: left-side covariant representation}
	\end{equation}
то это отображение является представлением группы $G$,
которое мы будем называть
\AddIndex{левосторонним ковариантным представлением}
{left-side covariant representation}.
		\end{theorem}
		\begin{proof}
Так как $f$ - гомоморфизм групп, то $f(e)=\delta$.

Согласно
\eqref{eq: left-side covariant product of transformations}
и \eqref{eq: left-side covariant representation}
\[
f(ab)u=(f(a)f(b))u=f(a)(f(b)u)
\]

Согласно определению \ref{definition: left-side representation of group}
$f$ является представлением.
		\end{proof}

		\begin{theorem}
		\label{theorem: right-side covariant representation}
Пусть $r(M)$ - группа относительно умножения
	\begin{equation}
u(t_1t_2)=(ut_1)t_2
	\label{eq: right-side covariant product of transformations}
	\end{equation}
и $\delta$ - единица группы $r(M)$.
Если отображение
\eqref{eq: right-side representation of group}
является гомоморфизмом групп
	\begin{equation}
f(ab)=f(a)f(b)
	\label{eq: right-side covariant representation}
	\end{equation}
то это отображение является представлением группы $G$,
которое мы будем называть
\AddIndex{правосторонним ковариантным представлением}
{right-side covariant representation}.
		\end{theorem}
		\begin{proof}
Так как $f$ - гомоморфизм групп, то $f(e)=\delta$.

Согласно
\eqref{eq: right-side covariant product of transformations}
и \eqref{eq: right-side covariant representation}
\[
uf(ab)=u(f(a)f(b))=(uf(a))f(b)
\]

Согласно определению \ref{definition: right-side representation of group}
$f$ является представлением.
		\end{proof}

		\begin{theorem}
		\label{theorem: left-side contravariant representation}
Пусть $l(M)$ - группа относительно умножения
	\begin{equation}
(t_2t_1)u=t_1(t_2u)
	\label{eq: left-side contravariant product of transformations}
	\end{equation}
и $\delta$ - единица группы $l(M)$.
Если отображение
\eqref{eq: left-side representation of group}
является антигомоморфизмом групп
	\begin{equation}
f(ba)u=f(a)f(b)
	\label{eq: left-side contravariant representation}
	\end{equation}
то это отображение является представлением группы $G$,
которое мы будем называть
\AddIndex{левосторонним контравариантным представлением}
{left-side contravariant representation}.
		\end{theorem}
		\begin{proof}
Так как $f$ - антигомоморфизм групп, то $f(e)=\delta$.

Согласно
\eqref{eq: left-side contravariant product of transformations}
и \eqref{eq: left-side contravariant representation}
\[
f(ab)u=(f(b)f(a))u=f(a)(f(b)u)
\]

Согласно определению \ref{definition: left-side representation of group}
$f$ является представлением.
		\end{proof}

		\begin{theorem}
		\label{theorem: right-side contravariant representation}
Пусть $r(M)$ - группа относительно умножения
	\begin{equation}
u(t_2t_1)=(ut_1)t_2
	\label{eq: right-side contravariant product of transformations}
	\end{equation}
и $\delta$ - единица группы $r(M)$.
Если отображение
\eqref{eq: right-side representation of group}
является антигомоморфизмом групп
	\begin{equation}
f(ba)u=f(a)f(b)
	\label{eq: right-side contravariant representation}
	\end{equation}
то это отображение является представлением группы $G$,
которое мы будем называть
\AddIndex{правосторонним контравариантным представлением}
{right-side contravariant representation}.
		\end{theorem}
		\begin{proof}
Так как $f$ - антигомоморфизм групп, то $f(e)=\delta$.

Согласно
\eqref{eq: right-side contravariant product of transformations}
и \eqref{eq: right-side contravariant representation}
\[
uf(ab)=u(f(b)f(a))=(uf(a))f(b)
\]

Согласно определению \ref{definition: right-side representation of group}
$f$ является представлением.
		\end{proof}

	\begin{example}
Групповая операция определяет два различных представления на группе:
\AddIndex{левый сдвиг}{left shift, group}, который мы определяем равенством
\symb{L(a)b}0{left shift}
	\begin{equation}
b'=\ShowSymbol{left shift}=ab
	\label{eq: left shift}
	\end{equation}
и \AddIndex{правый сдвиг}{right shift, group}, который мы определяем равенством
\symb{R(a)b}0{right shift}
	\begin{equation}
b'=\ShowSymbol{right shift}=ba
	\label{eq: right shift}
	\end{equation}
	 \qed
	 \end{example}

		\begin{theorem}
Пусть представление
	\[
u'=f(a)u
	\]
является ковариантным представлением. Тогда представление
	\[
u'=h(a)u=f(a^{-1})u
	\]
является контравариантным представлением.
		\end{theorem}
		\begin{proof}
Утверждение следует из цепочки равенств
\[h(ab)=f((ab)^{-1})=f(b^{-1}a^{-1})=f(b^{-1})f(a^{-1})=h(b)h(a)\]
		\end{proof}

	 \begin{definition}
Пусть $f$ - представление группы $G$ в множестве $M$.
Для любого $v\in M$ мы определим
\AddIndex{орбиту представления группы $G$}
{orbit of representation of group} как множество
\symb{\mathcal O(v,g\in G,f(g)v)=\{w=f(g)v:g\in G\}}2
{orbit of representation of group}
	 \qed
	 \end{definition}

Так как $f(e)=\delta$, то $v\in\mathcal{O}(v,g\in G,f(g)v)$.

		\begin{theorem}
		\label{theorem: proper definition of orbit}
Если
	\begin{equation}
	\label{eq: orbit, proposition}
v\in\mathcal{O}(u,g\in G,f(g)u)
	\end{equation}
то
\[
\mathcal{O}(u,g\in G,f(g)u)=\mathcal{O}(v,g\in G,f(g)v)
\]
		\end{theorem}
		\begin{proof}
Из \eqref{eq: orbit, proposition} следует
существование $a\in G$ такого, что
	\begin{equation}
v=f(a)u
	\label{eq: orbit, 1}
	\end{equation}
Если $w\in\mathcal{O}(v,g\in G,f(g)v)$, то
существует $b\in G$ такой, что
	\begin{equation}
w=f(b)v
	\label{eq: orbit, 2}
	\end{equation}
Подставив \eqref{eq: orbit, 1} в \eqref{eq: orbit, 2}, мы получим
	\begin{equation}
w=f(b)(f(a)u)
	\label{eq: orbit, 3}
	\end{equation}
На основании \eqref{eq: left-side product of transformations}
из \eqref{eq: orbit, 3} следует,
что $w\in\mathcal{O}(u,g\in G,f(g)u)$.
Таким образом,
\[
\mathcal{O}(v,g\in G,f(g)v)\subseteq\mathcal{O}(u,g\in G,f(g)u)
\]

На основании \eqref{eq: inverse transformation}
из \eqref{eq: orbit, 1} следует,
что
	\begin{equation}
u=f(a)^{-1}v=f(a^{-1})v
	\label{eq: orbit, 4}
	\end{equation}
Равенство \eqref{eq: orbit, 4} означает, что
$u\in\mathcal{O}(v,g\in G,f(g)v)$ и, следовательно,
\[
\mathcal{O}(u,g\in G,f(g)u)\subseteq\mathcal{O}(v,g\in G,f(g)v)
\]
Это завершает доказательство.
		\end{proof}

		 \begin{theorem}
		 \label{theorem: direct product of representations}
Если определены представление $f_1$ группы $G$ в множестве $M_1$
и представление $f_2$ группы $G$ в множестве $M_2$,
то мы можем определить
\AddIndex{прямое произведение представлений
$f_1$ и $f_2$ группы}
{direct product of representations of group}
	\begin{align*}
f&=f_1\otimes f_2:G\rightarrow M_1\otimes M_2\\
f(g)&=(f_1(g),f_2(g))
	\end{align*}
		\end{theorem}
		\begin{proof}
Чтобы показать, что $f$ является представлением,
достаточно показать, что $f$ удовлетворяет определению
\ref{definition: left-side representation of group}.
\[f(e)=(f_1(e),f_2(e))=(\delta_1,\delta_2)=\delta\]
	\begin{align*}
f(ab)u&=(f_1(ab)u_1,f_2(ab)u_2)\\
&=(f_1(a)(f_1(b)u_1),f_2(a)(f_2(b)u_2))\\
&=f(a)(f_1(b)u_1,f_2(b)u_2)\\
&=f(a)(f(b)u)
	\end{align*}
		\end{proof}

			\section{Однотранзитивное представление}

	 \begin{definition}
Мы будем называть
\AddIndex{ядром неэффективности представления группы}
{kernel of inefficiency of representation of group} $G$
множество \[K_f=\{g\in G:f(g)=\delta\}\]
Если $K_f=\{e\}$, мы будем называть представление группы $G$
\AddIndex{эффективным}{effective representation of group}.
	 \qed
	 \end{definition}

		\begin{theorem}
Ядро неэффективности - это подгруппа группы $G$.
		\end{theorem}
		\begin{proof}
Допустим
$f(a_1)=\delta$ и $f(a_2)=\delta$. Тогда
\[f(a_1a_2)u=f(a_1)(f(a_2)u)=u\]
\[f(a^{-1})=f^{-1}(a)=\delta\]
		\end{proof}

Если действие не эффективно, мы можем перейти к эффективному,
заменив группой $G_1=G|K_f$,
пользуясь факторизацией по ядру неэффективности.
Это означает, что мы можем изучать только эффективное действие.

	 \begin{definition}
Мы будем называть представление группы
\AddIndex{транзитивным}{transitive representation of group},
если для любых $a, b \in V$ существует такое $g$, что
\[a=f(g)b\]
Мы будем называть представление группы
\AddIndex{однотранзитивным}{single transitive representation of group},
если оно транзитивно и эффективно.
	 \qed
	 \end{definition}

		\begin{theorem}	%однотранзитивное
Представление однотранзитивно тогда и только тогда, когда для любых $a, b \in V$
существует одно и только одно $g\in G$ такое, что $a=f(g)b$
		\end{theorem}

	 \begin{definition}
Мы будем называть пространство $V$
\AddIndex{однородным пространством группы}{homogeneous space of group} $G$,
если мы имеем однотранзитивное представление группы $G$ на $V$.
	 \qed
	 \end{definition}

		\begin{theorem}	%
		\label{theorem: single transitive representation of group}
Если мы определим однотранзитивное представление $f$ группы $G$ на многообразии $A$,
то мы можем однозначно определить координаты на $A$, пользуясь координатами на группе $G$.

Если $f$ - ковариантное представление, то $f(a)$ эквивалентно левому сдвигу $L(a)$ на группе $G$.
Если $f$ = контравариантное представление, то $f(a)$ эквивалентно правому сдвигу $R(a)$ на группе $G$.
		\end{theorem}
		\begin{proof}
Мы выберем точку $v\in A$
и определим координаты точки $w\in A$
как координаты преобразования $a$ такого, что $w=f(a) v$.
Координаты, определённые таким образом, однозначны
с точностью до выбора начальной точки $v\in A$,
так как действие эффективно.

Если $f$ - ковариантное представление, мы будем пользоваться записью
\[f(a)v=av\]
Так как запись
\[f(a)(f(b)v)=a(bv)=(ab)v=f(ab)v\]
совместима с групповой структурой, мы видим, что ковариантное представление $f$ эквивалентно левому сдвигу.

Если $f$ - контравариантное представление, мы будем пользоваться записью
\[f(a)v=va\]
Так как запись
\[f(a)(f(b)v)=(vb)a=v(ba)=f(ba)v\]
совместима с групповой структурой, мы видим, что контравариантное представление $f$ эквивалентно правому сдвигу.
		\end{proof}

		\begin{theorem}	%
		\label{theorem: shifts on group commuting}
Левый и правый сдвиги на группе $G$ перестановочны.
		\end{theorem}
		\begin{proof}
Это следствие ассоциативности группы $G$
\[(L(a) R(b))c = a(cb)=(ac)b=(R(b) L(a))c\]
		\end{proof}

		\begin{theorem}	%
		\label{theorem: two representations of group}
Если мы определили однотранзитивное представление $f$ на многообразии $A$,
то мы можем однозначно определить однотранзитивное представление $h$
такое, что диаграмма
	\[
\xymatrix{
M\ar[rr]^{h(a)}\ar[d]^{f(b)} & & M\ar[d]^{f(b)}\\
M\ar[rr]_{h(a)}& &M
}
	\]
коммутативна для любых $a$, $b\in G$.\footnote{Теорема
\ref{theorem: two representations of group}
на самом деле очень интересна. Тем не менее её
смысл становится более ясным, когда мы приложим эту теорему к многообразию базисов,
смотри секцию \ref{section: Basis in Vector Space}.}
		\end{theorem}
		\begin{proof}
Мы будем пользоваться групповыми координатами для точек $v\in A$.
Для простоты мы предположим, что $f$ - ковариантное представление.
Тогда согласно теореме \ref{theorem: single transitive representation of group}
мы можем записать левый сдвиг $L(a)$ вместо преобразования $f(a)$.

Пусть точки $v_0, v\in A$. Тогда мы можем найти
одно и только одно $a\in G$ такое, что
\[v=v_0 a=R(a) v_0\]
Мы предположим
\[h(a)=R(a)\]
Существует $b\in G$ такое, что
\[w_0=f(b)v_0=L(b) v_0\ \ \ \ w=f(b)v=L(b) v\]
Согласно теореме \ref{theorem: shifts on group commuting} диаграмма
	\begin{equation}
\xymatrix{
v_0\ar[rr]^{h(a)=R(a)}\ar[d]^{f(b)=L(b)} & & v\ar[d]^{f(b)=L(b)}\\
w_0\ar[rr]_{h(a)=R(a)}& &w
}
	\label{Diagram: two representations of group}
	\end{equation}
коммутативна.

Изменяя $b$ мы получим, что $w_0$ - это произвольная точка, принадлежащая $A$.

Мы видим из диаграммы, что, если $v_0=v$ than $w_0=w$ и следовательно $h(e)=\delta$.
С другой стороны, если $v_0\neq v$, то $w_0\neq w$ потому, что представление $f$ однотранзитивно.
Следовательно представление $h$ эффективно.

Таким же образам мы можем показать, что для данного $w_0$ мы можем найти $a$
такое, что $w=h(a)w_0$. Следовательно представление однотранзитивно.

В общем случае, представление $f$ не коммутативно и следовательно
представление $h$ отлично от представления $f$.
Таким же образом мы можем создать представление $f$, пользуясь представлением $h$.
		\end{proof}

		\begin{remark}
		\label{remark: one representation of group}
Очевидно, что преобразования $L(a)$ и $R(a)$
отличаются, если группа $G$ неабелева.
Тем не менее, они являются отображениями на.
Теорема \ref{theorem: two representations of group} утверждает, что, если оба
представления правого и левого сдвига существуют на многообразии $A$,
то мы можем определить два перестановочных представления на многообразии $A$.
Только левый или правый сдвиг не может представлять оба типа представления.
Чтобы понять почему это так, мы можем изменить диаграмму \eqref{Diagram: two representations of group}
и предположить $h(a)v_0=L(a)v_0=v$ вместо $h(a)v_0=R(a)v_0=v$ и
проанализировать, какое выражение $h(a)$ имеет в
точке $w_0$. Диаграмма
\[\xymatrix{
v_0\ar[rr]^{h(a)=L(a)}\ar[d]^{f(b)=L(b)} & & v\ar[d]^{f(b)=L(b)}\\
w_0\ar[rr]_{h(a)}& &w
}\]
эквивалентна диаграмме
\[\xymatrix{
v_0\ar[rr]^{h(a)=L(a)} & & v\ar[d]^{f(b)=L(b)}\\
w_0\ar[rr]_{h(a)}\ar[u]_{f^{-1}(b)=L(b^{-1})}& &w
}\]
и мы имеем $w=bv=bav_0=bab^{-1}w_0$. Следовательно
\[h(a)w_0=(bab^{-1})w_0\] Мы видим, что представление $h$
зависит от его аргумента. \qed  
%There is interesting question. Если I имею преобразование $L(a)$ in точке $b$
%what is $c$ такое, что $L(a) b = R_c b$. Мы можем find it из равенства
%$ab=bc$, so $c=b^{-1}ab$, следовательно
%\[L(a) b = R_{b^{-1}ab} b\]?????
		\end{remark}

			\section{Линейное представление}

Если на множестве $M$ определена дополнительная структура,
мы предъявляем к представлению группы дополнительные требования.

Если на множестве $M$ определено понятие непрерывности,
то мы полагаем, что преобразование
	\[
u'=f(a)u
	\]
непрерывно по $u$
и, следовательно,
\[\left|\frac { \partial u'} {\partial u}\right|\neq 0\]

Если $M$ - группа, то большое значение имеют
представления левых и правых сдвигов.

	 \begin{definition}
Пусть $M$ - векторное пространство $\mathcal{V}$ над полем $F$.
Мы будем называть представление группы $G$ в векторном пространстве $\mathcal{V}$
\AddIndex{линейным представлением}
{linear representation of group},
если $f(a)$ - гомоморфизм пространства $\mathcal{V}$ для любого $a\in G$.
	 \qed
	 \end{definition}

		\begin{remark}
		\label{remark: row and column vectors, vector space}

Допустим, преобразование $f(a)$ является линейным
однородным преобразованием.
$f_\gamma^\beta(a)$ являются элементами матрицы
преобразования. Мы обычно полагаем, что нижний индекс
перечисляет строки в матрице и верхний индекс перечисляет столбцы.

Согласно закону умножения матриц мы можем
представить координаты вектора как строку матрицы.
Мы будем называть такой вектор
\AddIndex{вектор\hyph строкой}{row vector}.
Мы можем так же рассматривать вектор, координаты которого
формируют столбец матрицы и будем называть
такой вектор \AddIndex{вектор\hyph столбцом}{column vector}.

Левостороннее линейное представление в пространстве вектор\hyph столбцов
\[
u'=f(a)u\ \ \ \ u'_\alpha=f_\alpha^\beta(a)u_\beta\ \ \ \ a\in G
\]
является ковариантным представлением
\[
u''_\gamma=f_\gamma^\beta(ba) u_\beta
=f_\gamma^\alpha(b)(f_\alpha^\beta(a) u_\beta)
=(f_\gamma^\alpha(b)f_\alpha^\beta(a)) u_\beta
\]

Левостороннее линейное представление в пространстве вектор\hyph строк
\[
u'=f(a)u\ \ \ \ u'^\alpha=f^\alpha_\beta(a)u^\beta\ \ \ \ a\in G
\]
является контравариантным представлением
\[
u''^\gamma=f^\gamma_\beta(ba) u^\beta
=f^\gamma_\alpha(b)(f^\alpha_\beta(a) u^\beta)
=(f^\alpha_\beta(a)f^\gamma_\alpha(b)) u^\beta
\]

Правостороннее линейное представление в пространстве вектор\hyph столбцов
\[
u'=uf(a)\ \ \ \ u'_\alpha=u_\beta f_\alpha^\beta(a)\ \ \ \ a\in G
\]
является контравариантным представлением
\[
u''_\gamma=u_\beta f_\gamma^\beta(ab)
=(u_\beta f_\alpha^\beta(a))f_\gamma^\alpha(b)
=u_\beta(f_\gamma^\alpha(b)f_\alpha^\beta(a)) 
\]

Правостороннее линейное представление в пространстве вектор\hyph строк
\[
u'=uf(a)\ \ \ \ u'^\alpha=u^\beta f^\alpha_\beta(a)\ \ \ \ a\in G
\]
является ковариантным представлением
\[
u''^\gamma=u^\beta f^\gamma_\beta(ab)
=(u^\beta f^\alpha_\beta(a))f^\gamma_\alpha(b)
=u^\beta(f^\alpha_\beta(a)f^\gamma_\alpha(b)) 
\]
		\qed
		\end{remark}

		\begin{remark}
		\label{remark: covariant and contravariant representations}
При изучении линейного представления
мы явно будем пользоваться тензорной записью.
Мы можем пользоваться только верхним индексом и записью $u^\bullet{}_\alpha^.$ вместо
$u_\alpha$. Тогда мы можем записать преобразование этого объекта в виде
\[u'{}^\bullet{}_\alpha^.=f^\bullet{}_\alpha^.{}_\bullet{}^\beta_. u^\bullet{}_\beta^.\]
Таким образом мы можем спрятать различие между ковариантным и
контравариантным представлениями. Эта сходство идёт
сколь угодно далеко.
		\qed
		\end{remark}


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%
\Symb{texBiring}%
   {$(^{\gi a}_{\gi b})$\hyph\CR квазидетерминант}%
   {a b CR quasideterminant definition}%
\Symb{texBiring}%
   {$(^{\gi a}_{\gi b})$\hyph \RC квазидетерминант}%
   {a b RC-quasideterminant definition}%
\Symb{texBiring}%
   {минор}%
   {A from b a}%
\Symb{texBiring}%
   {минор}%
   {A from columns T}%
\Symb{texBiring}%
   {минор}%
   {A from rows S}%
\Symb{texBiring}%
   {минор}%
   {A without column a}%
\Symb{texBiring}%
   {минор}%
   {A without columns T}%
\Symb{texBiring}%
   {минор}%
   {A without row b}%
\Symb{texBiring}%
   {минор}%
   {A without rows S}%
\Symb{texPolymodule}%
   {активное преобразование}%
   {active transformation}%
\Symb{texTypeBasis}%
   {аффинное пространство}%
   {affine space}%
\Symb{texBasis}%
   {аффинное пространство}%
   {An}%
\Symb{texBiring}%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb{texBiring}%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb{texBiring}%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb{texBiring}%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb{texVectorSpace}%
   {\dcr вектор}%
   {dcr vector}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of left shift, 1-Parameter Group}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift, 1-Parameter Group}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb{texVectorSpace}%
   {\drc вектор}%
   {drc vector}%
\Symb{texAffine}%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb{texPolymodule}%
   {пассивное преобразование}%
   {passive transformation}%
\Symb{texBiring}%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb{texBiring}%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb{texBiring}%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb{texBiring}%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb{texBiring}%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb{texDrcRepresentation}%
   {правый сдвиг}%
   {right shift}%
\Symb{texAlgebraBundle}%
   {\sT сдвиг}%
   {starT shift, group bundle}%
\Symb{texDrcRepresentation}%
   {левый сдвиг}%
   {Tstar shift}%
\Symb{texAlgebraBundle}%
   {\Ts сдвиг}%
   {Tstar shift, group bundle}%
\Symb{texReferenceFrame}%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb{texReferenceFrame}%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%
\Symb{texBasis}%
   {многообразие базисов аффинного пространства}%
   {BAn}%
\Symb{texReferenceFrame}%
   {многообразие базисов многообразия}%
   {basis manifold of manifold}%
\Symb{texPolymodule}%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb{texBasis}%
   {многообразие базисов векторного пространства $\mathcal{V}$}%
   {basis manifold of vector space}%
\Symb{texBasis}%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb{texBasis}%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb{texTypeBasis}%
   {многообразие базисов аффинного пространства}%
   {FAn}%
\Symb{texTypeBasis}%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb{texTypeBasis}%
   {многообразие базисов евклидова пространства}%
   {FEn}%

\SetIndexSpace%
\Symb{texBasis}%
   {центро-аффинное пространство}%
   {CAn}%
\Symb{texTypeBasis}%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb{texLie}%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb{texLie}%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Symb{texReferenceFrame}%
   {множество функций, определённых на многообразии}%
   {set of functions defined on manifold}%

\SetIndexSpace%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of starT representation}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of starT representation, coordinates}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation, coordinates}%
\Symb{texVectorSpace}%
   {\dcr векторное пространство \subs строк}%
   {c rows dcr vector space}%
\Symb{texCalculus}%
   {дифференциал функции}%
   {differential, drc vector space to drc vector space}%
\Symb{texCalculus}%
   {дифференциал функции}%
   {differential, drc vector space to skew field}%
\Symb{texVectorSpace}%
   {\drc координатное векторное пространство}%
   {drc coordinate vector space}%
\Symb{texVectorSpace}%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb{texAffine}%
   {производная Картана}%
   {overbrace D}%
\Symb{texAffine}%
   {производная}%
   {overline D}%
\Symb{texCalculus}%
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 1, drc vector space}%
\Symb{texCalculus}%
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 1, skew field}%
\Symb{texVectorSpace}%
   {\drc векторное пространство \sups строк}%
   {r rows drc vector space}%
\Symb{texTidal}%
   {скорость отклонения}%
   {speed of deviation}%
\Symb{texVectorSpace}%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%
\Symb{texTypeBasis}%
   {аффинный базис}%
   {Affine Basis}%
\Symb{texBasis}%
   {аффинный базис}%
   {Affine Basis}%
\Symb{texTypeBasis}%
   {базис}%
   {basis}%
\Symb{texBasis}%
   {базис векторного пространства}%
   {Basis e}%
\Symb{texBasis}%
   {базис в векторном пространстве $\mathcal{V}$}%
   {basis in V}%
\Symb{texVectorSpace}%
   {базис в векторном пространстве}%
   {basis, vector space}%
\Symb{texPolymodule}%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb{texAlgebraBundle}%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb{texAlgebraBundle}%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb{texBasis}%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb{texReferenceFrame}%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb{texTypeBasis}%
   {евклидово пространство}%
   {En}%
\Symb{texBasis}%
   {евклидово пространство}%
   {En}%
\Symb{texBasis}%
   {псевдоевклидово пространство}%
   {Enm}%
\Symb{texTypeBasis}%
   {псевдоевклидово пространство}%
   {Enm}%
\Symb{texAlgebraBundle}%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb{texBasis}%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb{texAlgebraBundle}%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb{texAlgebraBundle}%
   {множество невырожденных \sT преобразований расслоения $\mathcal{E}$}%
   {set of starT nonsingular transformations of bundle}%
\Symb{texAlgebraBundle}%
   {множество невырожденных \Ts преобразований расслоения $\mathcal{E}$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb{texBasis}%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb{texReferenceFrame}%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb{texReferenceFrame}%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb{texReferenceFrame}%
   {векторное поле системы отсчёта}%
   {vector field, reference frame}%
\Symb{texBasis}%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%
\Symb{texVectorSpace}%
   {координаты базиса в \dcr векторном пространстве \subs строк}%
   {basis coordinates, c rows dcr vector space}%
\Symb{texVectorSpace}%
   {координаты базиса в \drc векторном пространстве \sups строк}%
   {basis coordinates, r rows drc vector space}%
\Symb{texVectorSpace}%
   {базис в \dcr векторном пространстве \subs строк}%
   {basis, c rows dcr vector space}%
\Symb{texVectorSpace}%
   {базис в \drc векторного пространства \sups строк}%
   {basis, r rows drc vector space}%
\Symb{texDiffEq}%
   {центро-аффинный}%
   {Central Affine Basis}%
\Symb{texReferenceFrame}%
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Symb{texAlgebraBundle}%
   {гомоморфизм расслоенных алгебр}%
   {homomorphism of algebra bundles}%
\Symb{texBundleRelation}%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb{texBundleRelation}%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb{texAlgebraBundle}%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb{texDrcRepresentation}%
   {орбита представления группы $G$}%
   {orbit of representation of group}%
\Symb{texTypeBasis}%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb{texReferenceFrame}%
   {система отсчёта}%
   {reference frame}%
\Symb{texReferenceFrame}%
   {система отсчёта}%
   {reference frame, extensive definition}%
\Symb{texPolymodule}%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb{texPolymodule}%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%
\Symb{texVectorSpace}%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb{texLie}%
   {алгебра Ли группы Ли}%
   {g}%
\Symb{texLie}%
   {определённая слева алгебра Ли группы Ли}%
   {gl}%
\Symb{texTypeBasis}%
   {группа аффинных преобразований}%
   {GLAn}%
\Symb{texBasis}%
   {группа аффинных преобразований}%
   {GLAn}%
\Symb{texLie}%
   {определённая справа алгебра Ли группы Ли}%
   {gr}%
\Symb{texBasis}%
   {группа гомоморфизмов векторного пространства $\mathcal{V}$}%
   {GV}%
\Symb{texDrcRepresentation}%
   {орбита ковариантного эффективного \sT представления группы}%
   {orbit of effective starT covariant representation of group}%
\Symb{texAlgebraBundle}%
   {орбита ковариантного эффективного \sT представления расслоенной группы}%
   {orbit of effective starT covariant representation of group bundle}%
\Symb{texDrcRepresentation}%
   {орбита ковариантного эффективного		\Ts представления группы}%
   {orbit of effective Tstar covariant representation of group}%
\Symb{texAlgebraBundle}%
   {орбита ковариантного эффективного		\Ts представления расслоенной группы}%
   {orbit of effective Tstar covariant representation of group bundle}%
\Symb{texVectorSpace}%
   {\RC матричная группа}%
   {rc-matrix group}%

\SetIndexSpace%
\Symb{texBiring}%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Symb{texLinearMap}%
   {\rcd векторное пространство \drc линейных отображений}%
   {rcd vector space of drc linear maps}%

\SetIndexSpace%
\Symb{texLieRepresentation}%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
\Symb{texLinearLie}%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%

\SetIndexSpace%
\Symb{texRepresentation}%
   {левый сдвиг}%
   {left shift}%
\Symb{texDiffProperty}%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb{texDiffProperty}%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb{texBasis}%
   {пассивное преобразование}%
   {passive transformation}%
\Symb{texRepresentation}%
   {множество левосторонних невырожденных преобразований множества $M$}%
   {set of left-side nonsingular transformations}%

\SetIndexSpace%
\Symb{texDrcRepresentation}%
   {множество невырожденных \sT преобразований множества $M$}%
   {set of starT nonsingular transformations}%
\Symb{texDrcRepresentation}%
   {множество невырожденных \Ts преобразований множества $M$}%
   {set of Tstar nonsingular transformations}%

\SetIndexSpace%
\Symb{texBasis}%
   {геометрический объект в координатном представлении}%
   {geometrical object, coordinate vector space}%
\Symb{texBasis}%
   {геометрический объект}%
   {geometrical object, vector space}%
\Symb{texRepresentation}%
   {орбита представления группы $G$}%
   {orbit of representation of group}%
\Symb{texAlgebraBundle}%
   {орбита представления расслоенной группы $\mathcal{G}$}%
   {orbit of representation of group bundle}%

\SetIndexSpace%
\Symb{texAlgebraBundle}%
   {расслоение}%
   {bundle}%
\Symb{texAlgebraBundle}%
   {декартова степень расслоения}%
   {Cartesian power of bundle}%
\Symb{texAlgebraBundle}%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb{texAlgebraBundle}%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb{texAlgebraBundle}%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb{texAlgebraBundle}%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%
\Symb{texBasis}%
   {активное преобразование}%
   {active transformation}%
\Symb{texAffine}%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb{texVectorSpace}%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in reduced bundle, 2}%
\Symb{texAffine}%
   {кривизна}%
   {GLn curvature_overline}%
\Symb{texVectorSpace}%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb{texRepresentation}%
   {правый сдвиг}%
   {right shift}%
\Symb{texRepresentation}%
   {множество правосторонних невырожденных преобразований множества $M$}%
   {set of right-side nonsingular transformations}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb{texBundleRelation}%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb{texBundleRelation}%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb{texVectorSpace}%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%

\SetIndexSpace%
\Symb{texLie}%
   {касательная плоскость к группе $G$}%
   {TaG}%

\SetIndexSpace%
\Symb{texBasis}%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb{texBasis}%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb{texVectorSpace}%
   {\dcr векторное пространство}%
   {left CR vector space}%
\Symb{texVectorSpace}%
   {\drc векторное пространство}%
   {left RC vector space}%
\Symb{texLinearMap}%
   {($S$, $T$)\hyph бимодуль}%
   {R S bimodule}%
\Symb{texVectorSpace}%
   {\crd векторное пространство}%
   {right CR vector space}%
\Symb{texVectorSpace}%
   {\rcd векторное пространство}%
   {right RC vector space}%
\Symb{texBasis}%
   {векторное пространство}%
   {V}%
\Symb{texReferenceFrame}%
   {векторное пространство векторных полей}%
   {vector space of vector fields}%

\SetIndexSpace%
\Symb{texPolymodule}%
   {геометрический объект в координатном представлении,		определённом в векторном пространстве}%
   {geometrical object, coordinate vector space}%
\Symb{texPolymodule}%
   {геометрический объект в векторном пространстве}%
   {geometrical object, vector space}%

\SetIndexSpace%
\Symb{texReferenceFrame}%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in bundle, 1}%

\SetIndexSpace%
\Symb{texTidal}%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb{texDrcRepresentation}%
   {тождественное преобразование}%
   {identical transformation}%
\Symb{texRepresentation}%
   {тождественное преобразование}%
   {identical transformation}%
\Symb{texBasis}%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb{texBiring}%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%
\Symb{texReferenceFrame}%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb{texAffine}%
   {символ Картана}%
   {Cartan symbol}%
\Symb{texAffine}%
   {связность}%
   {conection overline}%
\Symb{texAffine}%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb{texAlgebraBundle}%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%
\Symb{texLie}%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb{texLie}%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%
\Symb{texReferenceFrame}%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%

\SetIndexSpace%
\Symb{texReferenceFrame}%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb{texCalculus}%
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 2, drc vector space}%
\Symb{texCalculus}%
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 2, skew field}%
\Symb{texReferenceFrame}%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%

\SetIndexSpace%
\Symb{texLie}%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%
\Symb{texAffine}%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb{texAffine}%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb{texAffine}%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%
\Symb{texAlgebraBundle}%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb{texAlgebraBundle}%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb{texAlgebraBundle}%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb{texAlgebraBundle}%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb{texBundleRelation}%
   {подрасслоение}%
   {subbundle}%

\CloseIndex

